A Comprehensive Review for MRF and CRF Approaches in Pathology Image Analysis

Pathology image analysis is an essential procedure for clinical diagnosis of many diseases. To boost the accuracy and objectivity of detection, nowadays, an increasing number of computer-aided diagnosis (CAD) system is proposed. Among these methods, random field models play an indispensable role in improving the analysis performance. In this review, we present a comprehensive overview of pathology image analysis based on the markov random fields (MRFs) and conditional random fields (CRFs), which are two popular random field models. Firstly, we introduce the background of two random fields and pathology images. Secondly, we summarize the basic mathematical knowledge of MRFs and CRFs from modelling to optimization. Then, a thorough review of the recent research on the MRFs and CRFs of pathology images analysis is presented. Finally, we investigate the popular methodologies in the related works and discuss the method migration among CAD field.

==> ack.tex <==
\section*{Acknowledgements}
This work is supported by the ``National Natural Science Foundation of China'' (No. 61806047), 
the ``Fundamental Research Funds for the Central Universities'' (No. N2019003) 
and the ``China Scholarship Council'' (No. 2018GBJ001757). 
We thank Miss Zixian Li and Mr. Guoxian Li for their importantsupport and discussion in this work.
